Policy Transfer across Visual and Dynamics Domain Gaps via Iterative Grounding

The ability to transfer a policy from one environment to another is a promising avenue for efficient robot learning in realistic settings where task supervision is not available. This can allow us to take advantage of environments well suited for training, such as simulators or laboratories, to learn a policy for a real robot in a home or office. To succeed, such policy transfer must overcome both the visual domain gap (e.g. different illumination or background) and the dynamics domain gap (e.g. different robot calibration or modelling error) between source and target environments. However, prior policy transfer approaches either cannot handle a large domain gap or can only address one type of domain gap at a time. In this paper, we propose a novel policy transfer method with iterative "environment grounding", IDAPT, that alternates between (1) directly minimizing both visual and dynamics domain gaps by grounding the source environment in the target environment domains, and (2) training a policy on the grounded source environment. This iterative training progressively aligns the domains between the two environments and adapts the policy to the target environment. Once trained, the policy can be directly executed on the target environment. The empirical results on locomotion and robotic manipulation tasks demonstrate that our approach can effectively transfer a policy across visual and dynamics domain gaps with minimal supervision and interaction with the target environment. Videos and code are available at https://clvrai.com/idapt .

==> survey/imitation.tex <==
\section{Imitation Learning}

\subsection{Learning from Demonstration}

\paragraph{BC~\citep{pomerleau1989alvinn}:}
Learning a policy that mimics the expert policy represented by expert demonstrations in a supervised learning manner. A behavioral cloning policy is trained to predict $a$ from $o$ given a dataset $D=\{o_i, a_i\}$.

\paragraph{ABM~\citep{siegel2020keep}:}
The problem setup is offline RL and it updates the prior $\pi(a|s)$ with adaptive weights, which depend on a learned value approximation for each data sample (i.e. higher prior for $(s, a)$ with high value and lower prior for $(s, a)$ with low value).

\paragraph{GAIL~\citep{ho2016generative}:}
Most well-known IRL method these days. A discriminator network learns to distinguish expert transitions from agent transitions. Then, a policy uses the discriminator output as a reward signal and learns to fool the discriminator, which means the agent trajectory becomes similar to the expert trajectory. Due to unstable adversarial training, it is not easy to train and requires some implementation hack, such as weight initialization with a BC policy and early stopping.

\paragraph{RPL~\citep{gupta2019relay}:}
From demonstrations, a high-level policy is learned to predict a sub-goal ($\pi_{high}(s_t, s_{t+w}) \rightarrow s_{t+W_l} \forall w \in [1,W_h]$) and a low-level policy is trained to reach a sub-goal ($\pi_{low}(s_t, s_{t+w}) \rightarrow a_t \forall w \in [1,W_l]$).
This hierarchical framework can be fine-tuned for the downstream task using RL.

\paragraph{IRIS~\citep{mandlekar2019iris}:}


\paragraph{GTI~\citep{mandlekar2020learning}:}


\paragraph{T-REX~\citep{brown2019extrapolating} and D-REX~\citep{brown2019better}:}
T-REX learns a reward function from demonstrations with ranking. The objective to learn a reward can be written as

\begin{align}
  \label{eq:ranking_loss}
  \mathcal{L}_{\theta} = -\mathbb{E}_{\tau_i < \tau_j \sim \mathcal{D}} \left[
    \
    \log \frac{\exp \sum_{s_t \in \tau_j}{f_{\phi}(s_{t})}}{\exp \sum_{s_t \in \tau_i}{f_{\phi}(s_{t})} + \exp \sum_{s_t \in \tau_j}{f_{\phi}(s_{t})} }
  \right].
\end{align}

D-REX extends T-REX by generating ranked demonstrations by perturbing an expert policy with increasing scales of noises.

\paragraph{UPN~\citep{srinivas2018universal}:}

\subsection{Learning from Observations}

\paragraph{BCO~\citep{torabi2018behavioral}:}
Behavioral Cloning from Observation first collects rollouts from random exploration and learns an inverse model $\hat{a} \sim f(s, s')$. Then, it uses the inverse model to predict action label between two consecutive states in a demonstration and trains a BC policy with the state and predicted action, $(s, \hat{a})$.

\paragraph{Zero-shot Visual Imitation~\citep{pathak*2018zeroshot}:}


\paragraph{GAIfO~\citep{torabi2018generative}:}
A variant of GAIL~\citep{ho2016generative} for learning from observations. Instead of discriminating an expert transition and agent transition $(s, a)$, GAIfO discriminates an expert effect and agent effect $(s, s')$.
\readlater{I did not understand the detail of theoretical derivation.}

\paragraph{IDDM~\citep{yang2019imitation}:} 
Minimize causal entropy of the policy with the GAIfO formulation to close the gap between LfD and LfO.
\readlater{I did not understand the detail of theoretical derivation.}


\subsection{One-shot Imitation Learning}

\paragraph{One-shot Imitation~\citep{duan2017one-shot,finn2017one-shot}:}


\paragraph{SILO~\citep{lee2019silo}:}


\subsection{Third-Person Imitation}
Generally, in third-person imitation, we assume no action label is available since a demonstration is collected from an agent different from the learner (robot).

\paragraph{Perceptual Rewards~\citep{sermanet2017rewards}:}
It learns a perceptual reward function by segmenting demonstrations into fixed (3-4) segments.

\paragraph{TCN~\citep{sermanet2018time}:}
Time-contrastive loss is used to learn a latent representation between demonstrator and agent that can be used for an IRL style reward. The main idea is simple but implementation requires a lot of hack, such as augment a dataset with randomly executed robot videos.

\paragraph{Context Translation~\citep{liu2018imitation}:}
It translates a human demo frame to robot demo frame.

\paragraph{DAML~\citep{yu2018aone,yu2018bone}:}
Domain-Adaptive Meta-Learning to translate a human video to a robot action sequence.

==> survey/offline_rl.tex <==
\section{Offline Reinforcement Learning}

\paragraph{SQIL~\citep{reddy2020sqil}:} 
Instead of learning a reward function from demonstration, this paper proposes to simply label +1 reward for transitions from demonstration and 0 reward for agent transitions and then train a policy with any off-policy RL. During training, a half of a mini-batch is sampled from expert transitions and another half is sampled from agent transitions. Hence, the agent tends to follow expert's trajectory and even it is off the expert's trajectory, it encourages to get back to an expert trajectory.

==> survey/sim2real.tex <==
\section{Sim2Real}

\paragraph{RCAN~\citep{james2018simtoreal}}
Learns mappings from random to canonical (simulation) images so that real world images can also be translated at test time.  Decouples randomization from policy learning and does not require any real world data. 

\paragraph{Dynamics Randomization~\citep{Peng_2018}}
Randomizing simulator dynamics during training so policies can generalize to new dynamics in real world.

\paragraph{GraspGAN~\citep{bousmalis2017using}}
Learns transformation from synthetic to real images with generative adversarial, task, and content loss.  Applies feature level domain adaptation on top of transformed images.

\paragraph{DANN~\citep{ganin2015domainadversarial}}
Domain-Adversarial Neural Networks.  Given labeled source domain data and unlabeled target domain data, learn transferable policy through features that are informative about main learning task but uninformative for domain.

\paragraph{SimOpt~\citep{chebotar2018closing}}
Learn a simulation parameter distribution for domain randomization by minimizing the discrepancy between real world observation trajectories and simulated observation trajectories.

\paragraph{Visual Domain Randomization~\citep{tobin2017domain}}
Randomizing simulation rendering for object localization in real world cluttered environment.

\paragraph{Deep Visuomotor Policy~\citep{zhu2018reinforcement}}
Training model-free visuomotor policy by using Hybrid IL/RL Reward and Leveraging Physical States in Simulation. Sim2Real Policy Transfer by doing domain randomization

\paragraph{MATL~\citep{Wulfmeier2017mutual}}
Given sim and real have the same state space and only the underlying dynamics are different. Use discriminator to generate a alignment reward to match the trajectories between sim and real. 

\paragraph{Inverse dynamics model~\citep{Malmir2020Robust}}
While training in simulation, learn a inverse dynamics model that, given two state observation, predicts the action taken in-between. In real environment, compare the predicted action by inverse dynamics model and the actual action taken, and according to the discrepancy between the two, add a disturbance to the next action.

\paragraph{CuNAS~\citep{Hochreiter2020Long}}
Before training, learn a LSTM that predicts the discrepancies between sim and real by exploring the environment with Goal Babbling. Then, during training, the LSTM model is used to update the simulator at every state.

\paragraph{Incremental Learning~\citep{Josifovski2020Continual}}
The agent learn incrementally from low-realism to high-realism and in the end learn in the real world

\paragraph{Imitating Animal~\citep{peng2020learning}}
Retarget source motions to robot's morphology using IK, then train a RL policy to reproduce the motion in simulation. Then, use domain adaptation to transfer to a real robot.

\paragraph{V2R via Visual Semantic Segmentation~\citep{Hong2018V2R}}
Trains a perception module that learns meta-states to guide the downstream RL control policy. The perception module takes as input RGB images and output states, which goes to control policy module. Then, the policy will react with an action. A visual-guidance module can be incorporated to adjust the meta-state to alter the behavior of the robot online.

\paragraph{Manipulate Deformable Objects without Demonstrations~\citep{Wu2020Deform}}

\paragraph{Iterative Design for Sim-to-Real~\citep{Xie2019Cassie}}


\paragraph{Closing Sim-to-Real Gap~\citep{chebotar2018closing}}

Jason's sim2real paper

==> text/v0/approach_v0.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/training_simple.pdf}
    \caption{
        Our iterative environment grounding method alternates between two stages: (1)~source environment grounding and (2)~policy training. We ground the source environment in the target environment by learning a visual (purple) and action (yellow) transformations. During the grounding stage, we first train the visual transformation on unpaired images, and then train the action transformation.  During policy training, we fix the grounded environment and optimize the policy using RL.
    }
    \label{fig:training}
\end{figure*}


\section{Approach}

In this paper, we aim to address the problem of transferring a policy from a well-instrumented and controlled environment to a target environment with minimal information (\ie no reward and state information). However, in many robotics setups, policies trained in the source environment struggle at performing the learned task in the target environment due to the visual domain shift and dynamics changes. To overcome such domain gaps, we introduce a novel policy transfer method with iterative grounding. The key goal is to learn grounding a source environment so that a policy trained in this grounded environment can then directly execute in the target environment.
%to alternate between grounding both domain gaps and training a policy in the grounded environment, as illustrated in \myfigref{fig:training}.


%Our iterative environment grounding method is outlined in \mysecref{sec:iterative_domain_alignment}. The details of the two stages are elaborated in \mysecref{sec:grounded_environment} and \mysecref{sec:policy_training}.

% Our method consists of five components:
% \begin{itemize}
%     \item \textbf{Target environment}: is an environment to deploy a robot, which provides minimal information (\ie no state and reward information). 
%     \item \textbf{Source environment}: is an environment with easier access to reward and state information. This environment can have visual or physical differences from the target environment.
%     \item \textbf{Policy}: is defined on the state and action spaces of the target environment.    
%     \item \textbf{Visual transformation}: receives an image observation from the source environment and translates it to the corresponding target domain observation, which compensates for the visual domain gap between the two environments.
%     \item \textbf{Action transformation}: receives an observation and action from the target domain, and produces a source-domain action, which makes the source environment have the same transition with the target environment.
% \end{itemize}
% The grounded environment is composed of the source environment, visual transformation, and action transformation.




\subsection{Problem Formulation}
\label{sec:problem_formulation}

We consider an RL framework for policy transfer of a task from a source environment $S$ to target environment $T$.  The task is defined by a shared state space $\mathcal{S}$, action space $\mathcal{A}$, and reward function $\mathcal{R}: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$.  The source and target environments have different visual observation spaces, $\mathcal{O}^S$ and $\mathcal{O}^T$, and transition functions, $\mathcal{T}^S: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ and $\mathcal{T}^T: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$, respectively.  Note that the source environment provides full access to state $s^S$, reward $r^S$, and visual observation $o^S$ while the target environment only provides visual observations $o^T$.  Given a time horizon $H$ and discount factor $\gamma \in [0,1]$, our objective is to learn the optimal visual policy $\pi^*(a_t|o^T_t)$ that maximizes the expected return in the target environment:  
\begin{equation}
    \label{eqn:target_J}
    J(\pi) = \mathbb{E}_{\tau \sim p(\tau|\pi,\mathcal{T}^T )} \left [\sum_{t=0}^H \gamma^t r_t \right ].
\end{equation}
Due to the differences in observations and transition functions, this is not equivalent to maximizing the expected return in the source environment and results in different policies.

In addition, we assume access to task-agnostic datasets of unpaired visual observations in both domains, $\mathcal{D}_o^S = \{(o_t^S, s_t^S), (o_{t+1}^S, s_{t+1}^S), \cdots \}$ and $\mathcal{D}_o^T = \{o_t^T, o_{t+1}^T, \cdots \}$. These task-agnostic datasets do not need to align well with the current task, and therefore they can be collected via autonomous exploration, hand-specified calibration sequences, or policies trained for other tasks.  However, we assume the datasets share similar underlying state distributions.



\subsection{Iterative Environment Grounding}
\label{sec:iterative_domain_alignment}
To overcome domain gaps in policy transfer, our goal is to develop a novel policy transfer method with iterative grounding that alternates between (1) learning to ground the source environment in the target environment both visually and physically; and (2) learning a policy in this grounded environment, as illustrated in \myfigref{fig:training}:
\begin{itemize}
    \item \textbf{Source environment grounding}: we learn a \textit{visual transformation} and \textit{action transformation} that compensate for the visual and dynamics domain gaps between the two environments from unpaired trajectories.
    \item \textbf{Policy training}: the grounded environment acts as a proxy for the target environment, providing interactions with reward to train a policy.
\end{itemize}
%As illustrated in \myfigref{fig:training}, our method consists of two alternating stages: grounded environment learning and policy training. We call every complete pass through both stages a \textit{grounding step}. 

We first initialize the grounded environment by training the visual and dynamics transformations from unpaired, task-agnostic datasets. From the second grounding step, we collect task-relevant trajectories using the learned policy to improve the transformations. For every environment grounding, we further adapt our policy to the improved grounded environment.
%As can be seen in \myfigref{fig:result_step}, we found that one grounding step is enough for handling small domain gaps but five grounding steps are required for large domain gaps.
Since we do not have access to paired data, the transformations for grounding are trained with the unpaired, sub-optimal data. However, as the policy generates sub-optimal yet task-relevant data, the visual and dynamics transformations become more accurate around the task-relevant state and action spaces. The improved grounding makes the policy transfer better as the grounded environment can simulate the target environment better. Therefore, we iterate over these two stages to gradually improve the alignment between the grounded and target environments and the performance of the policy. The entire training procedure is outlined in \myalgref{alg:method}.


\subsection{Learning to Ground Environment}
\label{sec:grounded_environment}

%Due to the domain gaps, na\"ive policy transfer often fails to perform the task in the target environment~\citep{jakobi1995noise, peng2018sim, tobin2017domain}. For successful transfer of a policy, we can minimize the domain gaps by modifying the training (source) environment to produce similar trajectories as the testing (target) environment~\citep{hanna2017grounded, golemo2018sim}. Concretely, 
The goal of this step is to ground the source environment \textit{both visually and physically} using unpaired source and target environment trajectories. 
%, so that the grounded environment can be used to train a policy.
As the grounded environment is closer to the target environment, the policy trained in the grounded environment transfers better than the one trained in the original source environment.
%As the policy is trained in an environment that is more similar to the target environment, it transfers better than the one trained in the original source environment.

As illustrated in \myfigref{fig:training} (right), our grounded source environment is composed of three components: the source environment $S$, visual transformation $G: \mathcal{O}^S \rightarrow \mathcal{O}^T$, and action transformation $F: \mathcal{O}^T \times \mathcal{A} \rightarrow \mathcal{A}$. 
With these transformations, we ground the source environment by:
\begin{enumerate}[label=(\arabic*)]
\item Translating the source observation to the target domain, $\hat{o}_t^T = G(o_t^S)$.
\item Translating the target action to the source action to compensate dynamics mismatches, $\hat{a}_t^S = F(\hat{o}_t^T, a_t^T)$.
\item Rolling out the source environment, $o_{t+1}^S = ENV^S(o_t^S, \hat{a}_t^S)$. 
\item Translating the next source observation to the target domain, $\hat{o}_{t+1}^T = G(o_{t+1}^S)$. 
\end{enumerate}
Through this process, the grounded environment can simulate the target environment by taking $a_t^T$ and providing $\hat{o}_{t+1}^T$. In addition, this grounded environment can provide the task reward $\hat{r}_t^T = r_t^S$, which is not available in the target environment.

To achieve a transferable policy, it is crucial for the grounded environment to simulate the target environment as closely as possible. In the rest of this section, we explain how to efficiently learn accurate grounding by learning a visual transformation and action transformation from limited target environment data.


\subsubsection{\textbf{Learning Visual Transformation}} 
\label{sec:visual_transformation}

To transfer a visual policy, the visual domains of training and testing should be similar. To match the domains, we ground the source environment to be visually similar to the target environment by learning a visual transformation $G$. 

The visual transformation is first initialized using the task-agnostic datasets $\{\mathcal{D}_o^S, \mathcal{D}_o^T\}$, and then we iteratively improve it with online datasets $\{\mathcal{D}^S_{online}, \mathcal{D}^T_{online}\}$ collected using the current policy.  This serves to improve the transformation in the task-relevant observation spaces which may not be well represented in the initial datasets.

We train our visual transformation using an unsupervised image-to-image translation method, CycleGAN~\citep{zhu2017unpaired}, which optimizes the cycle-consistency loss between two domains. However, due to the lack of correspondences, the resulting visual transformation can map semantically incorrect images, \eg change the arrangements of objects in the scene.
To ensure the state information is preserved across domains (\ie the domains are semantically aligned), we propose a \textit{state reconstruction regularization}, which encourages the source state and the predicted state from the translated observation to be similar. Note that the state reconstruction can be replaced with any self-supervision, such as a robot state or reward.

Since the target environment does not provide the state information, a state predictor for the target observation cannot be trained. Instead, we train a source state predictor $s = P^{S}(o^{S})$ using the source domain dataset $\mathcal{D}_o^S$ with state labels, and generate pseudo-labeled target domain dataset $\{(G(o^S), s)|(o^S, s) \in \mathcal{D}_o^S \}$ to train the target state predictor $s = P^{T}(o^{T})$. Using this target state predictor, we can compute the state reconstruction regularization loss $\lVert P^{T}(G(o^{S})) - s \rVert_1$. We can jointly train the visual transformation and target state predictor by optimizing the CycleGAN objective with state reconstruction regularization:
\begin{equation}
\begin{aligned}
    \label{eqn:visual_loss}
    \mathcal{L}_{visual} &= \mathcal{L}_{CycleGAN}(o^{S}, o^{T}) + \lambda \lVert P^{T}(G(o^{S})) - s \rVert_1,
\end{aligned}
\end{equation}
where $\lambda$ a weighting factor for the regularization. For correct visual alignment, we encourage the state predictors to extract the shared state information: we initialize the target state predictor with the weights of the source state predictor and finetune only the top layer (\texttt{conv1}) in the target domain~\citep{aytar2017crossmodal, jeong2020selfsupervised}, as illustrated in \myfigref{fig:visual_transformation}.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/garat_model.png}
%     \caption{
%         Action transformation agent produces actions $a^S$ from observations $(s,a^T)$ to follow dynamics demonstrations gathered in the target environment.
%         To tackle image-based tasks, we utilize the visual transformation and a shared visual encoder($f(o)$) to extract domain-aligned features as a proxy for state
%     }
%     \label{fig:garat}
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/visual_transformation.pdf}
    \caption{
        To train the visual transformation, we first train the source state predictor (left bottom) with image-state pairs from the source environment, and copy its weights to the target state predictor. Then, we train image translation models (purple) and the first layer (\texttt{conv1}) of the target state predictor jointly using the CycleGAN loss and state reconstruction regularization.
    }
    \label{fig:visual_transformation}
\end{figure}


\subsubsection{\textbf{Learning Action Transformation}}
\label{sec:action_transformation}

In addition to the visual domain gap, physical domain gaps (\eg friction, mass, robot calibration) hinder transferring a policy to the target domain.  To deal with the discrepancy between the dynamics of the source and target environments, we learn an action transformation~\citep{hanna2017grounded, desai2020stochastic, karnan2020reinforced, desai2020imitation} that compensates for the dynamics mismatch.
We learn the action transformation $F(a^{S}|o^T,a^{T})$ from a target domain observation-action pair to a source domain action such that the resulting transition in the respective domains is the same.  This grounds the training environment in the target environment's dynamics, and thus a policy trained in the grounded environment can generate the same trajectories in the target environment.  

However, prior grounded action transformation approaches require access to a shared, low-dimensional state space across domains and are not suited for visual observations with domain gaps. Since our goal is to solve more realistic cases where the target environment does not provide access to such information, we extend the grounded action transformation to image observations with visual domain differences.  In this paper, we propose the use of visual features $f_\pi(o^T)$ generated by the policy network (\ie output of the convolutional layers of the policy network) as a proxy for the state since the policy extracts low-dimensional representations that contain task-relevant information.  Since $f_\pi$ is trained on the target domain we can directly use it to encode target domain observations into proxy states.  In the source domain, we can use the visual transformation $G$ to obtain the corresponding target domain observation. Hence, we can use $f_\pi$ to extract proxy states for both source and target domain observations.

To efficiently learn an action transformation on our proxy state representation, we use the state-of-the-art grounded action transformation method, GARAT~\citep{desai2020imitation} -- which requires only a few target domain trajectories -- by framing our problem as a demonstration-efficient imitation learning from observation problem in the source environment.  Specifically, the action transformation, recast as the agent, transforms actions between domains such that the resulting transitions in the source environment resemble the transitions gathered in the target environment, thereby correcting for any dynamics differences.  
%To handle visual inputs from different environments, we replace a state $s$ with $f_\pi(o^T)$ for the target domain and $f_\pi(G(o^S))$ for the source domain. 
We implement GARAT using GAIfO~\citep{torabi2018generative} and PPO~\citep{PPO}.


\begin{algorithm}[t]
    \caption{Policy transfer via iterative grounding}
    \label{alg:method}
    \begin{algorithmic}[1]
        \STATE \textbf{Input:} Task-agnostic dataset $\{\mathcal{D}_o^S,\mathcal{D}_o^T\}$, number of grounding steps $N$
        \STATE Randomly initialize policy $\pi$ and visual transformation $G$
        \STATE Initialize action transformation $F$ as identity function
        \STATE Pretrain source state predictor $P^S$ on $\mathcal{D}^S_o$
        \STATE Optimize $G$ with $P^T$ to minimize \myeqref{eqn:visual_loss} on $\{ \mathcal{D}^S_o, \mathcal{D}^T_o \}$
        \FOR {$i = 1,2,\cdots,N$}
            \STATE Optimize $\pi$ in grounded environment with RL 
            \STATE Roll out $\pi$ in target environment to obtain $ \mathcal{D}^T_{online}$
            \STATE Roll out $\pi$ in grounded environment to obtain $ \mathcal{D}^S_{online}$
            \STATE Finetune $P^S$, $G$, and $P^T$ on $\{\mathcal{D}^S_{online},\mathcal{D}^T_{online}\}$
            \STATE Optimize $F$ with GARAT on $\mathcal{D}^T_{online}$
        \ENDFOR
        \STATE \textbf{Output:} Policy $\pi$ to deploy in target environment
    \end{algorithmic}
\end{algorithm}  


\subsection{Policy Training}
\label{sec:policy_training}

With the grounded environment, a policy $\pi(a^T | o^T)$ can be trained using any RL algorithm as if it is trained on the target environment. The policy learns to maximize the expected return  from the grounded environment:
\begin{equation}
    \label{eqn:grounded_J}
    \hat{J}(\pi) = \mathbb{E}_{\tau \sim p(\tau| F(G, \pi \circ G),\mathcal{T}^S )} \left [\sum_{t=0}^H \gamma^t \hat{r}_t \right ].
\end{equation}
In this work, we use Asymmetric SAC~\citep{pinto2017asymmetric} for policy training, a variant of SAC~\citep{haarnoja2018sac} that is efficient for learning an image-based policies by using state-conditioned critics.  For each grounding step, we train the policy with 1k grounded environment steps.

Even though the policy only learns from the grounded source environment interactions, we can directly execute this policy on the target environment as our learned transformations effectively close the domain gaps between the source and target environments. This makes our method well suited for cases where task supervision is not available and data collection is expensive or dangerous in the target environment. Instead, our method efficiently learns the source environment grounding using a few target domain interactions, and then trains a policy by fully utilizing rich, cheaply obtained data from the well instrumented and controlled source environment.

The grounded environment trained with the task-agnostic dataset can be not accurate enough to learn a transferable policy. 
Hence, we improve the grounded environment using the task-relevant data collected using the updated policy, and then train the policy again using the better grounded environment. We iterate these two stages to gradually improve the grounded environment and the policy. The entire training procedure is outlined in \myalgref{alg:method}.



==> text/v0/experiments_v0.tex <==
\section{Experiments}

In this paper, we propose a policy transfer method with iterative grounding across visual and dynamics domains without task supervision in the target environment. Our method iteratively learns visual and action transformations with limited target environment data; uses these transformations to ground the source environment such that it emulates the target environment; and then trains a transferable policy in the grounded environment with rewards from the source environment.

Through our experiments, we aim to answer the following questions: (1)~Can our method effectively transfer a policy across visual and dynamics differences with minimal target environment information? (2)~How does our method scale to wider domain gaps when compared to prior work?  (3)~Can the iterative training process overcome poor initial datasets?


\subsection{Experimental Setup}

To test how well our method transfers a policy with various visual and physical domain gaps, we design two benchmark target environments, one with smaller domain gaps (Target-easy) and one with larger domain gaps (Target-hard), on five simulation-to-simulation transfer tasks: classic inverted pendulum, two locomotion, and two robotic manipulation tasks. We vary both physical parameters and visual appearances for the source and target environments.  The changes are summarized in \mytbref{tab:dynamics-diff} and \myfigref{fig:tasks}.  

For the evaluation metric of a policy transfer, we use the normalized target domain performance (reward or success rate).  For all methods and tasks, we report the average target environment performance and standard deviation over 5 random seeds unless otherwise stated.

%  We also report the normalized performance based on the target domain performance of a policy trained in the source environment as the lower bound and the target domain performance of a policy trained in the target environment as the upper bound. 
% We train our method for one grounding step for the easy target environment and five grounding steps for the hard target environment.  In each grounding step, we roll out the current policy in the target environment to gather 1k samples, for a total of 5k target environment samples across all grounding steps.  We then train the observation and action transformations each for a fixed number of epochs.  In the policy training stage, we train the policy in the grounded environment for a fixed number of environment interactions.  The transfer performance is evaluated in the target environment at the end of the policy training stage for every grounding step.  


\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{\linewidth}
        \centering
        \makebox[0.27\linewidth]{Source}
        \makebox[0.27\linewidth]{Target-easy}
        \makebox[0.27\linewidth]{Target-hard}
    \end{subfigure}
    \\
    \vspace{0.3em}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.27\linewidth]{figures/tasks/pendulum_source.png}
        \includegraphics[width=0.27\linewidth]{figures/tasks/pendulum_target.png}
        \includegraphics[width=0.27\linewidth]{figures/tasks/pendulum_target_hard.png}
        \caption{InvertedPendulum}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.27\linewidth]{figures/tasks/halfcheetah_source.png}
        \includegraphics[width=0.27\linewidth]{figures/tasks/halfcheetah_target.png}
        \includegraphics[width=0.27\linewidth]{figures/tasks/halfcheetah_target_hard.png}
        \caption{HalfCheetah}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.27\linewidth]{figures/tasks/walker_source.png}
        \includegraphics[width=0.27\linewidth]{figures/tasks/walker_target.png}
        \includegraphics[width=0.27\linewidth]{figures/tasks/walker_target_hard.png}
        \caption{Walker2d}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.27\linewidth]{figures/tasks/fetchreach_source.png}        
        \includegraphics[width=0.27\linewidth]{figures/tasks/fetchreach_target.png}        
        \includegraphics[width=0.27\linewidth]{figures/tasks/fetchreach_target_hard.png}
        \caption{Fetch-Reach}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.27\linewidth]{figures/tasks/sawyer_source.png}        
        \includegraphics[width=0.27\linewidth]{figures/tasks/sawyer_target.png}        
        \includegraphics[width=0.27\linewidth]{figures/tasks/sawyer_target_hard.png}
        \caption{Sawyer-Push}
    \end{subfigure}
    \caption{
        Visualize source domain (left) and target domains with small (middle) and large (right) domain gaps. While the target-easy environments slightly differ in color and lighting condition, the target-hard environments include drastic changes in camera viewpoint, texture, and background. Especially in the manipulation tasks, we use the Unity3D rendering engine to make the target-hard environments look more realistic. 
    }
    \label{fig:tasks}
\end{figure}


\subsection{Method \& Baselines}

To provide baselines for policy transfer performance, we evaluate multiple representative policy transfer methods that can handle visual and dynamics domain gaps as following:
\begin{itemize}
    \item \textbf{Robust RL} trains a policy by injecting additive Gaussian noise to the action space and augmenting images with random crop and color jitter~\citep{laskin2020reinforcement}. % This method does not require a modifiable simulator and can be applied easily on top of any RL method.  
    % For RL training, we use asymmetric SAC~\citep{pinto2017asymmetric}.

    \item \textbf{Domain Randomization (DR)}~\citep{tobin2017domain, peng2018sim} learns robust policies by randomizing the source environment's visual and dynamics parameters, including color, texture, lighting, viewpoint, friction, and armature. In order to provide a fair comparison, we define the randomization ranges to include both source and target environments (\textbf{DR-Wide}). For the cases where the DR policy is unable to learn to cover the full range, we also include a policy trained with a smaller randomization range (\textbf{DR-Narrow}). % The implementation details about domain randomization can be found in appendix, \mysecref{sec:dr_implementation}.

    \item \textbf{Learning Cross-Domain Correspondence (CC)}~\citep{zhang2021learning} utilizes a learned state-to-visual observation mapping and an action mapping to transfer a policy across input modalities and dynamics domains. We train CC with a dataset of 50k images in either domain, following the original experimental setup in ~\citet{zhang2021learning}.  Note that CC does not transfer a visual policy in the source domain but transfers a state-based policy to obtain a visual policy in the target environment.
    
    \item \textbf{Our Method} takes iterative grounding steps where we collect target environment data to update our grounded environment and policy, as described in \mysecref{sec:iterative_domain_alignment}. For these experiments, we start out with a dataset of 20k images from either domain and additionally collect 1k target environment samples per grounding step.  We execute 5 grounding steps for target-hard environments and 1 grounding step for target-easy environments.  
    
\end{itemize}



\begin{table}[t]
\centering
\begin{tabular}{ ccccc } 
 \toprule
 \multirow{2}{7.5em}{\centering Task} & \multirow{2}{6.5em}{\centering Parameter} & \multirow{2}{3em}{\centering Source} & \multicolumn{2}{c}{Target} \\ 
 & & & Easy & Hard \\
 \midrule
 InvertedPendulum & Pendulum mass & 4.895 & 50 & 200 \\ 
 \midrule
 HalfCheetah & Armature & 0.1 & 0.18 & 0.4 \\ 
 \midrule
 Walker2d & Torso mass & 3.534 & 5.4 & 10.0 \\ 
 \midrule
 \multirow{2}{7.5em}{\centering Fetch-Reach} & Action Rotation & 0 & 30 & 45$^{\circ}$\\
 & Action Bias & 0 & 0 & -0.5 \\
 \midrule
 Sawyer-Push & Puck mass & 0.01 & 0.03 & 0.05 \\
 \bottomrule
\end{tabular}
\vspace{1em}
\caption{Dynamics differences between source and the two target domains.  We chose different physical parameters to vary for each environment that would affect transfer performance.}
\label{tab:dynamics-diff}
\end{table}


\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.75\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/all_comparisons/all_comparisons_legend.png}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/all_comparisons/all_comparisons_InvertedPendulum.png}
        \caption{InvertedPendulum}
        \label{fig:result_step:invertedpendulum}
    \end{subfigure}
    \begin{subfigure}[t]{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/all_comparisons/all_comparisons_HalfCheetah.png}
        \caption{HalfCheetah}
        \label{fig:result_step:halfcheetah}
    \end{subfigure}
    \begin{subfigure}[t]{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/all_comparisons/all_comparisons_Walker2d.png}
        \caption{Walker2d}
        \label{fig:result_step:walker2d}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/all_comparisons/all_comparisons_Fetch-Reach.png}
        \caption{Fetch-Reach}
        \label{fig:result_step:fetchreach}
    \end{subfigure}
    \begin{subfigure}[t]{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/all_comparisons/all_comparisons_Sawyer-Push.png}
        \caption{Sawyer-Push}
        \label{fig:result_step:sawyer_push}
    \end{subfigure}
    \begin{subfigure}[t]{0.29\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/visual_ablation/visual_ablation_Walker2d.png}
        \caption{Walker2d (Ablation)}
        \label{fig:ablation}
    \end{subfigure}
    \caption{
    Performance of policies when evaluated in the target-hard domain.  (a-e) We report success rates for manipulation tasks and reward for other tasks. The baseline methods do not take online target environment interactions so we report their final evaluation performance after training.  (f) Ablation of our action transformation (over 3 random seeds). We evaluate the mean performance over 100 episodes for all methods. The results with normalized rewards can be found in appendix, \myfigref{fig:result_step_norm}.
    }
    \label{fig:result_step}
\label{fig:exps}
\end{figure*}


\subsection{Inverted Pendulum}

We first examine the InvertedPendulum task, which is a classic continuous control task~\citep{brockman2016openai}. We create the target environments by changing the pendulum mass,  color, and background color. For the target-hard environment, we make these changes more significant and tilt the camera angle and the background texture. We collect trajectories of 20k images by taking random actions for the task-agnostic dataset.

\myfigref{fig:result_all:invertedpendulum} shows that our method outperforms baseline methods in transferring to both target-easy and target-hard domains. Moreover, our method shows a high target data efficiency as it achieves nearly maximum reward starting from the first grounding step, as shown in \myfigref{fig:result_step:invertedpendulum}. 

We can also observe that DR-Narrow and DR-Wide achieve 60\% and 40\% success rates on the target-easy domain but fail to generalize to the target-hard domain.  Our results show that with the smaller randomization range, DR-Narrow learns the task well but fails to generalize beyond the training domain distribution. In contrast, DR-Wide is difficult to train as the resulting policy must learn to cover a large range of visual and physical domains; but once trained, it can perform better in the target environment with a large domain gap.

Note that the domain gaps both for the target-easy and target-hard environments are large enough that the Robust RL baseline performs as poorly as direct transfer of a policy trained in the source domain. With the Robust RL baseline, we can verify the difficulty of our experimental setup across all tasks.


\subsection{Locomotion}

HalfCheetah and Walker2d are two representative locomotion tasks~\citep{brockman2016openai}. For dynamics domain shifts, we vary the armature~\citep{zhang2021learning} and torso mass~\citep{desai2020imitation} for HalfCheetah and Walker2d, respectively. For the visual domain shifts of the target-easy environment, we make small changes in the agent and background color. For the target-hard environment, we create a domain gap in the visual style of DeepMind Control Suite~\citep{tassa2018deepmind} and change the camera viewpoint.

To study the effect of different datasets for initial visual transformation training for our method and correspondence training for CC, we collect two task-agnostic datasets, one using random actions and one with a policy trained to walk backwards. In the following results, we first compare absolute transfer performance by reporting the best performance out of the two datasets.  We then do an analysis on the effect of dataset quality in \mysecref{sec:dataset_analysis}.


% Similarly, the stable agent pose can make randomly collected data include diverse and meaningful behaviors, where CC can learn correspondences without need for additional data.

In the target-hard environment of HalfCheetah, DR-Wide performs better than our method (see \myfigref{fig:result_step:halfcheetah}) and CC achieves comparable results with ours.  We hypothesize that the stable agent pose and relative ease of the task can allow a policy to find conservative actions that work with a large range of dynamics. On the other hand, learning explicit domain correspondences can still have some errors, resulting in poorer policy performance.  CC also benefits from the stable agent pose because even task agnostic data can include diverse and meaningful behaviors for the task at hand.  Therefore, CC can learn the necessary correspondences for policy transfer without the need for additional data.

The Walker2D character is an example of a locomotion problem that is less stable and more prone to falling.  Here, we demonstrate the relative advantage of our method for more difficult control tasks where domain differences are more crippling.  Our method is able to achieve up to 75\% of the upper bound value \myfigref{fig:result_step_norm:walker2d} while the baselines cannot improve much beyond direct transfer.  In fact, the strongest baseline here is DR-Narrow, but it does not generalize well to the target-hard task outside of its training distribution.  In contrast, DR-Wide fails to learn a good policy for any domain because the randomization range required to fit the target environment is too challenging for this type of control task.

% Because our method learns an image to image translation, decoupled from the action transformation,


\begin{figure*}[t]
    \centering
    %\begin{subfigure}[t]{0.55\linewidth}
    \begin{subfigure}[t]{0.27\linewidth}    
        \includegraphics[width=\linewidth]{figures/results/domain_comparisons/domain_gap_comparisons_legend.png}
    \end{subfigure}
    \\
    % \begin{subfigure}[t]{0.49\linewidth}
    \begin{subfigure}[t]{0.19\linewidth}
        \includegraphics[width=\linewidth]{figures/results/domain_comparisons/domain_gap_comparisons_InvertedPendulum.png}
        \caption{InvertedPendulum}
        \label{fig:result_all:invertedpendulum}
    \end{subfigure}
    \begin{subfigure}[t]{0.19\linewidth}
    %\begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/results/domain_comparisons/domain_gap_comparisons_HalfCheetah.png}
        \caption{HalfCheetah}
        \label{fig:result_all:halfcheetah}
    \end{subfigure}
    %\\
    \begin{subfigure}[t]{0.19\linewidth}
    % \begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/results/domain_comparisons/domain_gap_comparisons_Walker2d.png}
        \caption{Walker2D}
        \label{fig:result_all:walker2d}
    \end{subfigure}
    \begin{subfigure}[t]{0.19\linewidth}
    % \begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/results/domain_comparisons/domain_gap_comparisons_Fetch-Reach.png}
        \caption{Fetch-Reach}
        \label{fig:result_all:fetch_reach}
    \end{subfigure}
    %\\
    \begin{subfigure}[t]{0.19\linewidth}
    % \begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/results/domain_comparisons/domain_gap_comparisons_Sawyer-Push.png}
        \caption{Sawyer-Push}
        \label{fig:result_all:sawyer_push}
    \end{subfigure}
    \caption{
        Performance of policies transferred to the target domains with different sized domain gaps. 
    }
\label{fig:domain_exps}
\end{figure*}


\subsection{Manipulation}

We evaluate our method in two robotic manipulation tasks with the 7-DoF Fetch robot: Fetch-Reach~\citep{plappert2018robotics} and the 7-DoF Rethink Sawyer robot: Sawyer-Push. The robot must move its end effector to a goal position in Fetch-Reach or push a puck to a target position for Sawyer-Push. For the target-easy domain, we simply change colors, lighting conditions, and viewpoint (Fetch-Reach only); but in the target-hard domain, we emulate a realistic visual gap by generating more realistic background and changing viewpoint using Unity3D.  The dynamics differences for Sawyer-Push come from puck mass and friction. In Fetch-Reach we bias and rotate the input actions to model calibration error.  For the initial target domain dataset, we collect 20k images from either domain with random end-effector control.

In Fetch-Reach, our method achieves greater than 90\% success rate in both domain gaps (see \myfigref{fig:result_all:fetch_reach}), demonstrating a robustness to a wide visual gaps.  The visual transformation can handle drastic changes in viewpoint and background, as well as the more realistic rendering.  In addition, we attain a good success rate in just one grounding step \myfigref{fig:result_step:fetchreach}, showing the effectiveness of our grounded environment with only a few target environment interactions.

In Sawyer-Push, our method achieves a 75\% success rate in five grounding steps while all other methods fail to reach the goal in the target-hard environment. This task is more difficult due to the wide visual domain gap as well as the varying mass of the object which can be hard to adapt to based on task-agnostic data.  The increasing learning curve in \myfigref{fig:result_step:sawyer_push} shows the benefit of iterative domain alignment: our method shows low performance for the first three grounding steps but as the visual and action transformations provide better grounding of the source environment, the policy successfully transfers to the target environment.  Moreover, in the initial dataset, the robot is very unlikely to have moved the puck, making it difficult for CC to model the puck dynamics and therefore fails to transfer a policy.  For our method, the initial visual transformation also suffers and fails to translate a moving puck's position correctly but is improved over multiple iterations as the transformation is finetuned over a better data distribution.  

% Sawyer-Push, adapted from \citet{yuke2020robosuite}, a 7-DoF Sawyer robot must learn how to push a cylindrical puck to a marked goal location.  The robot is actuated by end effector position control constrained to the plane of the tabletop.  To emulate a realistic visual gap, we use Unity3d rendering to generate the target domain images with more realistic background and lighting as well as viewpoint changes.  The dynamics differences are puck mass and friction. We collect the initial dataset of 20k images from either domain with random end effector control.

% Sawyer-Slide is adapted from \citet{valassakis2020crossing}.  In this task, the Sawyer robot operates in joint-velocity space and the end effector is attached to a cardboard plate.  The objective is to slide a rectangular puck on the plate to a goal location by tilting the plate.  Similar to the Sawyer-Push task, we use varying background, lighting, viewpoint, puck mass and friction, and gather 20k images using random end effector control.

% Fetch-Reach~\citep{plappert2018robotics} asks a 7-DoF Fetch robotics arm to move its end-effector to the target position.



\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.7\linewidth}        
        \includegraphics[width=\linewidth]{figures/results/dataset_comparisons/dataset_comparisons_legend.png}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/results/dataset_comparisons/dataset_comparisons_HalfCheetah.png}
        \caption{HalfCheetah}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/results/dataset_comparisons/dataset_comparisons_Walker2d.png}
        \caption{Walker2d}
    \end{subfigure}
    \caption{
        Performance of policies transferred to the target domain using initial datasets of different qualities.  ``Random" is collected by a random agent, ``Backwards" is collected by an agent trained to move in the backwards direction, and ``Expert" is collected by an expert agent on the current task.
    }
\label{fig:dataset_exps}
\end{figure}


\subsection{Effect of Initial Dataset Quality}
\label{sec:dataset_analysis}

One critical factor for domain adaptation is the quality of the data, specifically the relevance to the current task.  If the dataset does not align with the state distribution or behaviors of the current task, the learned correspondences may not generalize, and therefore fail to transfer a policy for the task.  We analyze the effect of dataset quality on the HalfCheetah and Walker2d tasks for our method and CC.  We use three different datasets, collected by a random policy (Random), a policy trained to move backwards (Backwards), and a policy trained on the current task (Expert).  Here, the Random and Backwards datasets do not align well with the task.  In all experiments, we use datasets of 20k images in both domains and 5 grounding steps and CC uses 50k images in both domains following its original experimental setup~\citep{zhang2021learning}.  We report the final transfer performance in terms of reward in \myfigref{fig:dataset_exps}.  With the exception of HalfCheetah Random data, our method consistently achieves better transfer than CC.  With our iterative training procedure we can obtain better task-aligned data through training, which mitigates the effects of a poor initial dataset.  In Walker2d, our method actually performs better with the Backwards dataset rather than the perfectly aligned Expert data.  The expert policy used for the experiment has little variability in its behavior, resulting in an image translation that does not generalize well to an imperfect agent.  Meanwhile, the backwards policy experienced a wide range of poses resulting in a more robust image translation for training that can be later improved.  While alignment of both datasets with the current task and the breadth of its distribution are key factors that affect the quality of a learned transformation, through iterative grounding, our method is able to overcome this issue.


\subsection{Ablation on Action Transformation}

To verify the importance of closing dynamics domain gaps, we compare the performance of our method with and without the action transformation.  In the ablated model, we only train the visual transformation during the grounding step and apply actions directly in each environment.  \myfigref{fig:ablation} shows that even without the action transformation, our method can achieve 0.5 normalized reward, whereas all baseline methods get 0. This shows the difficulty in generalizing to the visual domain of the target-hard environment and how well our method can bridge the visual domain gap using the visual transformation.
On the other hand, this ablated model demonstrates a large drop in performance compared to our full model, which quantifies the performance gains by correcting the dynamics gap. Furthermore, with the dynamics domain gap, the distribution of the target domain data can be far from the source domain data.  When this happens, the quality of the translation will not improve and can lead to worse transfer performance when dynamics differences are unaccounted for.  Thus, it is vital that our method addresses both visual and dynamics domain gaps for the full benefits of iterative grounding.

